AeonG: An Efficient Built-in Temporal Support in Graph Databases

Real world graphs are often dynamic and evolve over time. It is crucial for storing and querying graph evolution in graph databases. However, existing works either suffer from high storage overhead or lack efficient temporal query support, or both. In this paper, we propose AeonG, a new graph database with built-in temporal support. AeonG is based on a novel temporal graph model. To fit this model, we design a storage engine and a query engine. Our storage engine is hybrid, with one current storage to manage the most recent versions of graph objects, and another historical storage to manage the previous versions of graph objects. This separation makes the performance degradation of querying the most recent graph object versions as slight as possible. To reduce the historical storage overhead, we propose a novel anchor+delta strategy, in which we periodically create a complete version (namely anchor) of a graph object, and maintain every change (namely delta) between two adjacent anchors of the same object. To boost temporal query processing, we propose an anchor-based version retrieval technique in the query engine to skip unnecessary historical version traversals. Extensive experiments are conducted on both real and synthetic datasets. The results show that AeonG achieves up to 5.73X lower storage consumption and 2.57X lower temporal query latency against state-of-the-art approaches, while introducing only 9.74% performance degradation for supporting temporal features

==> extend_version/2_model.tex <==
\section{Modeling and query language}
\label{sec:background}

In this section, we formulate the temporal graph model and present the temporal query language used in {\tgdb}. 

\subsection{Temporal Property Graph Model}
\label{sec:graph_model}

We define the temporal graph model by extending the static property graph model \todo{\cite{property_graph, cypher,property_graph_model,pg-key}} with a time dimension.
In the property graph model, real-world entities are represented as \todo{nodes}, and the relationships between these entities are modeled as edges. Each \todo{node} or edge has a unique identifier (id for short), possibly several labels (e.g., customer, phone), and properties (e.g., Name: Jack).

\todo{
\begin{definition}[Property Graph]
\label{def:pgm}
% {\textbf (Property Graph Model)} 
Let $\mathcal{N}$ and $\mathcal{E}$ denote sets of node ids and edge ids, respectively. Assume countable sets $\mathcal{L}$, $\mathcal{K}$, and $\mathcal{V}$ of \textit{labels, property names}, and \textit{property values}. A property graph is a tuple $G=\langle N, E, \rho, \lambda, \pi \rangle$ where:
\begin{itemize}[leftmargin=*,itemsep=2pt,topsep=0pt,parsep=0pt]
\item $N$ is a finite subset of $\mathcal{N}$, whose elements are referred to as the \textit{nodes} of $G$;
\item $E$ is a finite subset of $\mathcal{E}$, whose elements are referred to as the \textit{edges} of $G$ and $N \cap E =\emptyset$;
\item $\rho$: $E$ $\to$ $(N \times N)$ is a total function mapping each edge to its source and destination nodes;
 \item $\lambda: (N \cup E) \rightarrow 2^{\mathcal{L}}$ is a total function mapping nodes and edges to finite sets of labels (including the empty set); 
\item $\pi:(N \cup E) \times \mathcal{K} \rightarrow \mathcal{V}$ is a finite partial function, mapping a node/edge and a property key to a value.
\end{itemize}
\end{definition}
}


The property graph model, originally designed for static graphs, lacks the inherent ability to capture the evolution of graphs over time. 
In the context of relational databases, the concept of ``Transaction Time''~\cite{sql-2011} is proposed to bring a time dimension to the relational model.
This transaction time is created and maintained by the database system itself, tracking the lifespan of each data item within the system.
Inspired by the transaction time, we integrate the time dimension into the property graph model to formally define the temporal property graph model.


\todo{
\begin{definition}[Temporal Property Graph]
\label{def:tpgm}
A temporal property graph is a tuple $G=\langle \Omega, N, E, \rho,\lambda, \pi, \sigma, \tau \rangle$ where:
\begin{itemize}[leftmargin=*,itemsep=2pt,topsep=0pt,parsep=0pt]
\item $\Omega$ is a temporal domain, which is a finite set of consecutive timestamps, that is, $\Omega=\{i\in T | a \leq i\leq b\}$ for some $a$, $b \in T$ such that $a \leq b$.
$T$ represents the universe of time points;
\item $N$, $E$, $\rho$, $\lambda$, $\pi$ inherit  their definitions from Definition \ref{def:pgm};
\item $\sigma: (N \cup E) \times \Omega \to \{true, false\} $ is a total function that maps a node or an edge and a time period $\omega$ to a Boolean variable, indicating whether this node or edge exists during period $\omega$;
\item $\tau:(N \cup E) \times \mathcal{K} \times \Omega \rightarrow \mathcal{V}$ is a partial function that maps a node or an edge and a property key, and a time period $\omega$ to a value.
\end{itemize}
\end{definition}
}

\todo{
\textbf{{Constraints.}} 
Two constraints are imposed on our temporal property graph model to enforce that the graph at any time point corresponds to a valid conventional property graph. At any time point $t$:  (1) An edge exists only if both source and destination vertices/nodes exist at $t$. Formally, if $e \in E$, $\sigma(e,t)=true$, and $\rho(e)=(v_1,v_2)$, then $\sigma(v_1,t)=true$ and $\sigma(v_2,t)=true$; (2) A property can only take on a value during the time period when the corresponding vertex or edge exists. Formally, if $\tau(o,k,t)=val$, where $ o\in(N \cup E)$, $k\in\mathcal{K}$, $val\in\mathcal{V}$, then $\sigma(o,t)=true$. 
}



\makesure{ In contrast to existing approaches that assign the time period to each vertex or edge (e.g., T-GQL~\cite{T-GQL}), our model assigns the time period to each version of a vertex or edge. A graph object (vertex or edge) may have one or more versions, each associated with $\omega$ to convey various semantics at different time periods. Such a design enables the collection of the evolution of a graph object, providing a less complex and more efficient model for managing temporal graph data.} At any given time $t$, a graph object version with $\omega=[st,ed)$ is said to be \textbf{{\visible}} if  $st\leq t<ed$. We classify a graph object version as a current version if it is legal at the current time, and
as a historical version if it is not legal at the current time.

\todo{
\textbf{{Graph operations.}} 
Our temporal model supports diverse graph operations as follows. Assume these graph operations are issued by a transaction committed at time $t_1$.
\begin{itemize}[leftmargin=*,itemsep=2pt,topsep=0pt,parsep=0pt]
\item \textit{Creating} a vertex or an edge: this involves adding a vertex or edge with 
a current version having a time period $\omega=[t_1, +\infty)$.
\item \textit{Deleting} a vertex or an edge whose current version is with $\omega=[st, +\infty)$: this entails updating $\omega$ to  $[st, t_1)$.
\item  \textit{Updating} a vertex or an edge whose current version is with $\omega=[st, +\infty)$: 
this marks the current version as a historical version by updating $\omega$ to $[st, t_1)$ and generates a new current version with $\omega=[t_1, +\infty)$ representing the up-to-date semantics. 
\end{itemize}
}


\begin{figure}[]
\centering    %居中
% \setlength{\abovecaptionskip}{0.3cm}
\includegraphics[width=0.45\textwidth]{figures/graph_model.pdf}
\centering
\vspace{-4mm}
\caption{Example of a temporal property graph}
% \vspace{-3mm}
%\vspace{-2mm}
\label{fig:exp_model}
\end{figure}

%对应graph model的时间，举例子
% \vspace{-2mm}
% \begin{example}
% \label{exp:tpgm}
\makesure{\textbf{Example 2.} 
According to Definition \ref{def:tpgm}, we present the corresponding temporal property graph of Example 1 in Figure \ref{fig:exp_model}. Here, $\Omega=[t_0, +\infty]$, $N=[ v_0, v_1, v_2, v_3]$, $E=[ e_0, e_1, e_2, e_3]$. Each vertex and edge owns a current version and several historical versions from $t_0$ to $t_n$. 
For brevity, we omit graphical states before $t_n$. At $t_n$, there exists three vertices ($v_0$, $v_1$ and $v_2$) and two edges ($e_0: (v_0,v_1))$ and $e_1:(v_0,v_2)$).
For instance, $v_2$ owns a current version $v_{2.7}$, which has 
a unique id $2$, a label ``Phone'', a property with the key-value pair (IP, Singapore), and a lifespan $\omega=[t_{n},\infty)$. 
Subsequently, at $t_{n+1}$, a customer purchase transaction takes place and changes the graph state. It updates the properties of $v_1$ and $v_2$, resulting in new versions for each of them. 
Take $v_2$ as an example: it marks $v_{2.7}$ as a historical version and generates a new current version $v_{2.8}$. Specifically, $\tau$ maps $v_{2.8} \times {IP} \times [t_{n+1},+\infty)$ to $\operatorname{\textit{New York}}$ and maps $v_{2.7} \times {IP} \times [t_{n},t_{n+1})$ to $\operatorname{\textit{Singapore}}$. Note $v_2$ is legal during the lifespan from $v_{2.0}$ to $v_{2.8}$. $\sigma$ maps $(v_2) \times [t_{0},+\infty)$ to $true$, indicating $v_2$ is created at $t_{0}$ and becomes {\visible} from then on.
Moreover, this transaction also creates $v_3$, $e_2$ and $e_3$, which all have only one current version with $\omega=[t_{n+1}, +\infty)$.
All the aforementioned graph operations adhere to the constraints we defined earlier. For instance, $e_2$ is successfully created at $t_{n+1}$ only after verifying that its linked vertices $v_3$ and $v_1$ are both {\visible} at $t_{n+1}$ (Constraint 1).  \qed
}

\subsection{Temporal Graph Query Language}
\label{sec:temporal_query_language}
{\tgdb} is designed to be an online system that inherently integrates temporal support.
Therefore, beyond basic queries such as creating, reading, updating, and deleting the current \makesure{versions}
% states 
of graph objects, {\tgdb} also excels at reading the historical 
\makesure{versions}
% states 
of graph objects.
This capacity empowers users to apply any time conditions to temporal queries,
spanning a wide time range from the oldest historical records up to the most recent updates.


{\tgdb} incorporates Cypher~\cite{cypher} as its query language and directly uses the existing Cypher syntax for data manipulation operations as introduced in Section \ref{sec:graph_model}. 
In addition, {\tgdb} extends the syntax of read queries to retrieve temporal graph data of user interest. 
\todo{As illustrated in Listing \ref{lst:cypher}, 
it introduces two syntax extensions within the \texttt{MATCH} clause of Cypher (line 3):}
% For fetching historical data, there are two syntax extensions introduced: 
(1) FOR $TT$ AS OF $t$, which retrieves all graph objects {\visible} at time $t$, and 
(2) FOR $TT$ FROM $t_1$ TO $t_2$, which locates all graph objects always {\visible} within the time range from $t_1$ to $t_2$. 
The former is referred to as ``time-point queries'', while the latter is known as ``time-slice queries''. 

\renewcommand\thelstlisting{\arabic{lstlisting}}

\begin{lstlisting}[mathescape,caption={Syntax extension on the Match Clause of Cypher},label={lst:cypher}, abovecaptionskip=0pt]
[OPTIONAL] MATCH pattern_tuple 
           [WHERE expr] 
           [FOR TT AS OF expr| FOR TT FROM expr TO expr]
\end{lstlisting}——

\textbf{Example 3.}
Consider the query ``What was Jack's phone IP and transaction location at $t_n${''}. This query can be answered by issuing the following Cypher-extended statement, where the underlined query statement represents the temporal syntax. 
% The underlined query statement represents the temporal syntax we have introduced, which bestows the query with the capacity to retrieve temporal graph data.
\vspace{-1mm}
$$
\begin{array}{l}
% \begin{align}{l}
% \begin{aligned}
\text { MATCH (n:Customer)-[r]-(p:Phone)-[:Messages]-(t:Transaction) } \\
\text { WHERE n.Name=`Jack' } \\
\text { \uline{FOT TT AS OF $t_n$ }} \\
\text { RETURN p.IP, t.Loc \quad \quad \quad \quad \quad \quad \quad \quad \qquad \qquad \qquad \quad \qed}
% \end{aligned}
% \end{align}
\end{array}
$$
% \end{example}
% \end{comment}

% MATH (x:Person{test=``pos"}) FOR TT AS OF 1 RETURN x \dotuline

% \uline{\textit{Query features.}}
% \textbf{{Query features.}} 
%设计目标是一个online 的查询; 可以支持current data, fresh historical data，old historical data.
% \vspace{-2mm}

% The time condition of a temporal query can be set at any desired time point, with a broad time range that spans from ancient records to the latest updates.
% by simply specifying the temporal conditions in the statements.


% and is capable of capturing not only current data but also historical data. We continually generate fresh historical data. So we are able to capture not only distant-past historical data but also recent-past historical data. 
% % One design goal of {\tgdb} is to support online queries. 
% % We are aimed to capture not only current data but also fresh/recent-past historical data and old/distant past historical data. 
% That is, the time condition of a temporal query can be set at any desired time point, providing a broad time range that spans from ancient records to the latest updates.

% (1) {\tgdb} focuses on accessing small portions of a graph.  {\tgdb} supports all the operations that are typically targeted by existing graph databases, but with the added capability of time travel in the time dimension. Analysis of current graph databases\cite{junghanns2017management} has shown that they primarily focus on OLTP-like CRUD operations for vertices and edges, as well as queries on smaller portions of a graph. For example, find all friends and interests of a user. {\tgdb} aligns with existing graph databases and includes this query feature.
% It is shown that current graph database systems mostly focus on queries on small portions of a graph, such as retrieving subgraphs or K-pop neighborhoods of specified nodes, for example, to find all friends and interests of a certain user.
% The analysis of current graph
% database systems in [42] showed that they mostly focus on
% OLTP-like CRUD operations (create, read, update, delete) for
% vertices and edges as well as on queries on smaller portions
% of a graph, for example, to find all friends and interests of a
% certain user.
% (2) The second notable feature of {\tgdb} is its ability to perform queries at any desired time point. {\tgdb} supports different time granularities, including the current time, the recent past, and the distant past. The data stored in {\tgdb} can range from ancient records to the latest updates, providing a wide temporal scope.

% long-past time period, the recent-past time period, and the current time period. The data can be as old as a fossil or as recent as the latest update. 
% Our system design should fit the above features.
% we aim to deal with different time granularity. The time of queries can be set at any point within a defined period, including the long-past time period, the recent-past time period, and the current time period. The data can be as old as a fossil or as recent as the latest update. Our system design should fit the above features.

% \textbf{Structural dimension.} First, we focus on accessing small portions of a graph with time dimension. It is showed that current graph database systems mostly focus on queries on small portions of a graph, such as retrieve subgraphs or k-pop neighborhoods of specified nodes. Based on this kind of queries, we explicitly reference temporal information to limit the time scope.
% %additionally introduce time dimension To explicitly reference temporal information, we additionally introduce time dimension on this kind of queries.


